Gated Multimodal Fusion with Contrastive Learning for Turn-taking Prediction in Human-robot Dialogue

Turn-taking, aiming to decide when the next speaker can start talking, is an essential component in building human-robot spoken dialogue systems. Previous studies indicate that multimodal cues can facilitate this challenging task. However, due to the paucity of public multimodal datasets, current methods are mostly limited to either utilizing unimodal features or simplistic multimodal ensemble models. Besides, the inherent class imbalance in real scenario, e.g. sentence ending with short pause will be mostly regarded as the end of turn, also poses great challenge to the turn-taking decision. In this paper, we first collect a large-scale annotated corpus for turn-taking with over 5,000 real human-robot dialogues in speech and text modalities. Then, a novel gated multimodal fusion mechanism is devised to utilize various information seamlessly for turn-taking prediction. More importantly, to tackle the data imbalance issue, we design a simple yet effective data augmentation method to construct negative instances without supervision and apply contrastive learning to obtain better feature representations. Extensive experiments are conducted and the results demonstrate the superiority and competitiveness of our model over several state-of-the-art baselines.

==> 05-related_work.tex <==
\section{Related work}
\label{sec:majhead}

The approaches of turn-taking can be summarized into three categories \cite{skantze2020turn}. (1) Silence-based models. Voice Active Detection (VAD) is usually used to detect if the user finished the speaking. A silence duration threshold is designed manually to decide when to take the turn. (2) IPU-based models. Tons of recent works \cite{local1986towards,edlund2005exploring,gravano2011turn,johansson2016making,liu2017turn,ishimoto2017end,roddy2018investigating,liu2019neural,ward2019prosodic,hara2019turn} belongs to this line because of its simplicity in practical applications. IPUs are first detected with VAD, then various multimodal cues including prosodic, semantic, linguistic, even visual features are extracted and integrated to determine whether the turn is yielded or not. (3) Continuous models. The user's speech is processed incrementally which allows the system to make continuous turn-taking decisions \cite{skantze2017towards,roddy2018investigating,ward2018turn,roddy2018multimodal}. However, it needs for revision as what the user is saying might change as more speech is being processed. Besides, the calculation efficiency can also be challenging to guarantee continuous processing.  

Our proposed approach belongs to IPU-based models. Different from previous works, we focus on a unified framework to fuse multimodal information seamlessly. Both endpointing and barge-in can be modelled with our proposed model. MFTP can also be easily extended if visual cues (e.g., gesture or eye-gaze) are available. Besides, Transformer and ResNet can also be upgraded to more advanced neural models in the future. 
